PIPER: Primitive-Informed Preference-based Hierarchical Reinforcement Learning via Hindsight Relabeling

In this work, we introduce PIPER: Primitive-Informed Preference-based Hierarchical reinforcement learning via Hindsight Relabeling, a novel approach that leverages preference-based learning to learn a reward model, and subsequently uses this reward model to relabel higher-level replay buffers. Since this reward is unaffected by lower primitive behavior, our relabeling-based approach is able to mitigate non-stationarity, which is common in existing hierarchical approaches, and demonstrates impressive performance across a range of challenging sparse-reward tasks. Since obtaining human feedback is typically impractical, we propose to replace the human-in-the-loop approach with our primitive-in-the-loop approach, which generates feedback using sparse rewards provided by the environment. Moreover, in order to prevent infeasible subgoal prediction and avoid degenerate solutions, we propose primitive-informed regularization that conditions higher-level policies to generate feasible subgoals for lower-level policies. We perform extensive experiments to show that PIPER mitigates non-stationarity in hierarchical reinforcement learning and achieves greater than 50$\%$ success rates in challenging, sparse-reward robotic environments, where most other baselines fail to achieve any significant progress.

==> figures_tex/explain_method.tex <==
\begin{figure*}
% \begin{minipage}{0.59\textwidth}
\centering
\captionsetup{font=footnotesize,labelfont=scriptsize,textfont=scriptsize}
\subfloat[][Maze navigation]{\includegraphics[scale=0.24]{figures/maze_alpha_success_rate.png}}
\subfloat[][Pick and place]{\includegraphics[scale=0.24]{figures/pick_alpha_success_rate.png}}
\subfloat[][Push]{\includegraphics[scale=0.24]{figures/push_alpha_success_rate.png}}
\subfloat[][Kitchen]{\includegraphics[scale=0.24]{figures/kitchen_alpha_success_rate.png}}
\\
% {\includegraphics[scale=0.5]{figures/legend_success.pdf}}
% \caption{\textbf{Learning rate $\alpha$ ablation} This figure compares the success rate performances for various values of primitive informed regularization weight $\alpha$ hyper-parameter. We choose these hyper-parameter values after extensive empirical comparisons. If the value of $\alpha$ is too small, we loose the advantages of primitive informed regularization, leading to degrading performance. In contrast, if the value of $\alpha$ is too large, it may lead to degenerate solutions. Thus, the variations in success rate performances demonstrate that proper primitive subgoal regularization is crucial for appropriate subgoal prediction, and improving overall performance.}
\label{fig:ablation_alpha}
\end{figure*}

==> figures_tex/kitchen_successful_viz.tex <==
\begin{figure}[H]
\vspace{5pt}
\centering
\captionsetup{font=footnotesize,labelfont=scriptsize,textfont=scriptsize}
\includegraphics[scale=0.1]{figures/kitchen_seed_6_viz_1.pdf}
\includegraphics[scale=0.1]{figures/kitchen_seed_6_viz_1.pdf}
\includegraphics[scale=0.1]{figures/kitchen_seed_6_viz_2.pdf}
\includegraphics[scale=0.1]{figures/kitchen_seed_6_viz_3.pdf}
% \includegraphics[scale=0.1]{figures/kitchen_seed_6_viz_3.pdf}
\includegraphics[scale=0.1]{figures/kitchen_seed_6_viz_4.pdf}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{\textbf{Successful visualization}: The visualization is a successful attempt at performing kitchen task}
\label{fig:kitchen_viz_success_2_ablation}
\end{figure}



==> figures_tex/maze_successful_viz.tex <==
\begin{figure}[H]
\vspace{5pt}
\centering
\captionsetup{font=footnotesize,labelfont=scriptsize,textfont=scriptsize}
\includegraphics[scale=0.11]{figures/maze_seed_5_viz_1.pdf}
\includegraphics[scale=0.11]{figures/maze_seed_5_viz_2.pdf}
\includegraphics[scale=0.11]{figures/maze_seed_5_viz_3.pdf}
\includegraphics[scale=0.11]{figures/maze_seed_5_viz_4.pdf}
\includegraphics[scale=0.11]{figures/maze_seed_5_viz_5.pdf}
\includegraphics[scale=0.11]{figures/maze_seed_5_viz_6.pdf}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{\textbf{Successful visualization}: The visualization is a successful attempt at performing maze navigation task}
\label{fig:maze_viz_success_2_ablation}
\end{figure}



==> figures_tex/pick_successful_viz.tex <==
\begin{figure}[H]
\vspace{5pt}
\centering
\captionsetup{font=footnotesize,labelfont=scriptsize,textfont=scriptsize}
\includegraphics[scale=0.11]{figures/pick_seed_3_viz_1.pdf}
\includegraphics[scale=0.11]{figures/pick_seed_3_viz_2.pdf}
\includegraphics[scale=0.11]{figures/pick_seed_3_viz_3.pdf}
\includegraphics[scale=0.11]{figures/pick_seed_3_viz_4.pdf}
\includegraphics[scale=0.11]{figures/pick_seed_3_viz_5.pdf}
\includegraphics[scale=0.11]{figures/pick_seed_3_viz_6.pdf}
\caption{\textbf{Successful visualization}: This figure provides visualization of a successful attempt at performing pick and place task}
\label{fig:pick_viz_success_2_ablation}
\end{figure}



==> figures_tex/push_successful_viz.tex <==
\begin{figure}[H]
\vspace{5pt}
\centering
\captionsetup{font=footnotesize,labelfont=scriptsize,textfont=scriptsize}
\includegraphics[scale=0.08]{figures/push_1.jpg}
\includegraphics[scale=0.08]{figures/push_2.jpg}
\includegraphics[scale=0.08]{figures/push_3.jpg}
\includegraphics[scale=0.08]{figures/push_4.jpg}
\includegraphics[scale=0.08]{figures/push_5.jpg}
\includegraphics[scale=0.08]{figures/push_6.jpg}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.jpg}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.jpg}
\caption{\textbf{Successful visualization}: The visualization is a successful attempt at performing push task}
\label{fig:push_viz_success_2_ablation}
\end{figure}



==> sections/old_method.tex <==
\section{Proposed Approach}


\subsection{Preference based Learning}
In traditional RL, agents learn to maximize the expected sum of environment rewards $r(s_t,a_t)$. However, in many scenarios, the environment rewards are notoriously difficult to construct, and require complex domain-specific knowledge. We consider Preference-based RL setup, where agent learns to perform a task using preferences over agent behaviors~\citep{NIPS2012_16c222aa, christiano2017deep, DBLP:journals/corr/abs-2106-05091, DBLP:journals/corr/abs-1811-06521}. The agent behaviors can be represented as a sequence $\delta^{i}$ of observations and actions: $\delta^{i}=((s_t^{i},a_t^{i}),(s_{t+1}^{i},a_{t+1}^{i})...(s_{t+k}^{i},a_{t+k}^{i}))$. The preferences encompass an underlying reward function $\widehat{r}_{\phi}$ with neural network parameters $\phi$, which is modeled using Bradley-Terry model~\citep{bradley_terry}:
\begin{equation}
\label{eqn:bradley_terry}
    P_\phi\left[\delta^1 \succ \delta^2\right]=\frac{\exp \sum_t \widehat{r}_\phi\left(\mathbf{s}_t^1, \mathbf{a}_t^1\right)}{\sum_{i \in\{1,2\}} \exp \sum_t \widehat{r}_\phi\left(\mathbf{s}_t^i, \mathbf{a}_t^i\right)}
\end{equation}
Here, $[\delta^1 \succ \delta^2]$ denotes that behavior sequence $\delta^1$ is preferred over sequence $\delta^2$. The behavior preference data is recorded in dataset $\mathcal{D}$, with entries of the form $(\delta^1, \delta^2, y)$. Here, $y=(1,0)$ when $\delta^1$ is preferred over $\delta^2$, $y=(0,1)$ when $\delta^2$ is preferred over $\delta^1$, and $y=(0.5,0.5)$ when both $\delta^1$ and $\delta^2$ are equally preferred. The reward function $\widehat{r}_{\phi}$ is learnt using following cross-entropy loss:
\begin{equation}
\label{eqn:reward_cross_entropy}
    \begin{split}
    & \operatorname{L}(\hat{r_{\phi}})=-\sum_{\left(\delta^1, \delta^2, y\right) \in \mathcal{D}} y(1) \log P_\phi\left[\delta^1 \succ \delta^2\right]+ 
    \\ & \hspace{3.35cm} y(2) \log P_\phi\left[\delta^2 \succ \delta^1\right]
    \end{split}
\end{equation}

\us{How does preference learning helps address these issues:\\ Issue 1. We propose to solve the non-stationarity in reward function, by replacing it with reward model $\widehat{r}_{\phi}$ learnt using preference based learning. This works as $\widehat{r}_{\phi}$ depends on current lower primitive behavior (as explained in PiL), which is dynamically updated, therefore reducing non-stationarity. \\ Issue 2. In order to predict achievable subgoals, we regularize the reward PiL $r^{s}$ with lower primitive value function for a behavior trajectory $\sigma$. The lower primitive value function $V(s_t, sg_t)$ will have a high value for subgoal $sg_t$, if it is achievable(or has been achieved already in the past). Thus, this regularization generates $r_{total}$, which is regularized reward for generating preferences.}

Outline:
\begin{itemize}
    \item Overview of PIPER approach
    \item Why should we expect a preference-based approach to be helpful in addressing aforementioned limitations of HRL? (e.g., learn a high-level reward for subgoal prediction; what else?)
    \item Why does preference-based fail? (e.g., cannot have humans relabel)
    \item Introduce PiL to overcome lack of human feedback
    \item PiL signal is too sparse, need to densify using HER
    \item PiL+HER must tailor subgoal difficulty, need to introduce value regularization
    \item Statement of PIPER approach
\end{itemize}


\label{sec:method}
In this section, we introduce our approach PIPER: \textbf{P}rimitive \textbf{I}n-the-loop \textbf{P}r\textbf{E}ference based hierarchical reinforcement learning via hindsight \textbf{R}elabeling for solving complex sparse reward tasks. Let $s$ be the current state, $sg$ be the subgoal predicted by higher level, and $g$ be the final goal. Formally, we represent the higher level policy $\pi^{H}(sg|s, g)$, higher level state value function $V^{H}(s,g)$, lower level primitive $\pi^{L}(a|s, sg)$, and lower level state value function $V^{L}(s,sg)$. In goal-conditioned HRL,  we represent the lower level primitive behavior as a sequence $\delta$ of states and primitive actions: $\delta^{i}=((s_t^{i},a_t^{i}),(s_{t+1}^{i},a_{t+1}^{i})...(s_{t+k}^{i},a_{t+k}^{i}))$, and the higher level primitive behavior as a sequence $\sigma$ of states and higher level actions (subgoal predictions): $\sigma^{i}=((s_t^{i},sg_t^{i}),(s_{t+k}^{i},sg_{t+k}^{i})...(s_{t+nk}^{i},sg_{t+nk}^{i}))$, where the higher level policy is executed for $n$ timesteps and lower primitive is executed for $k$ timesteps.

\subsection{PiL: Primitive-in-the-loop feedback}
\label{section:pil}
We first introduce our Primitive-in-the-loop (PiL) approach for generating higher level preference feedback. In standard preference based learning, the preferences are generated according to an implicit reward function $r:\mathcal{S}\times\mathcal{G}\times\mathcal{A}\rightarrow\mathcal{R}$. Let $g$ be the final goal and $\sigma^{1}$ and $\sigma^{2}$ be two higher level behavior sequences, where $\sigma^1 \succ \sigma^2$ implicitly implies:
\begin{equation}
\label{eqn:PiL}
    \begin{split}
        r(s_t^{1},g,sg_t^{1})+ r(s_{t+k}^{1},g,sg_{t+k}^{1})+...r(s_{t+nk}^{1},g,sg_{t+nk}^{1}) 
        & > \\ r(s_t^{2},g,sg_t^{2})+ r(s_{t+k}^{2},g,sg_{t+k}^{2})+...r(s_{t+nk}^{2},g,sg_{t+nk}^{2})
    \end{split}
\end{equation}
The preferences are elicited from human feedback~\cite{christiano2017deep} and are subsequently used to learn reward model $\widehat{r}_{\phi}$. In our work, we propose to replace Human-in-the-loop (HiL) feedback with Primitive-in-the-loop (PiL) feedback, by utilizing implicit sparse rewards $r^{s}(s_t,g,sg_{t})$ to determine preferences $y$ between behavior sequences $\sigma^{1}$ and $\sigma^{2}$. We call this feedback \textit{Primitive-in-the-loop} since we generate this feedback using primitive sparse rewards. Subsequently, we use the preference data $(\sigma^{1}, \sigma^{2}, y)$ to learn the reward model $\widehat{r}_{\phi}$, and use it to relabel the transitions in the higher level replay buffer.
\par Suppose the higher level policy $\pi^{H}$ predicts action $\pi^{H}(sg_t|s_t,g)$ for state $s_t$ and goal $g$. The lower level primitive executes primitive actions $\pi^{L}(a|s_t,sg_t)$ for $k$ timesteps and ends up in state $s_{t+k}$. We use the sparse reward  provided by the environment at state $s_{t+k}$ as the implicit sparse reward $r^{s}(s_t,g,sg_{t})=-1(\|s_{t+k}-g\|_2 > \epsilon)$. The reward $r^{s}$ is $0$ if we reach within $\epsilon$ distance of goal $g$ and $-1$ otherwise. Thus, $r^{s}$ elucidates the quality of subgoal prediction $\pi^{H}(sg_t|s_t,g)$. Note that this does not use any privileged information, as this sparse reward is directly available from the environment. We replace the implicit reward $r$ in Equation \ref{eqn:PiL} with $r^{s}$, and thus use $r^{s}$ to obtain preferences between higher level behavior sequences. Concretely, for the goal $g$, $\sigma^1 \succ \sigma^2$ when: 
\begin{equation}
\label{eqn:reward_s}
    \begin{split}
        \sum_{j=0}^{n} r^{s}(s_{t+jk}^{1},g,sg_{t+jk}^{1}) > \sum_{j=0}^{n} r^{s}(s_{t+jk}^{2},g,sg_{t+jk}^{2})
    \end{split}
\end{equation}
The preferences elicited using $r^{s}$ are subsequently used to learn the preference reward function $\widehat{r}_{\phi}$.
%
\was{Is $\widehat{r}_{\phi}$ being simply updated or entirely retrained at the end of each $k$-length trajectory?} \us{$\widehat{r}_{\phi}$ is simply updated here, but we also use target networks (Sec 3.4), which helps with training stability.}

\par Off-policy HRL approaches suffer from non-stationarity due to obsolete transitions in higher level replay buffer. The rewards in the higher level replay buffer transitions become obsolete due to changing lower level primitive. In our approach, the rewards in higher level replay buffer are relabeled using $\widehat{r}_{\phi}$. Hence, the transitions are updated from $(s_t, g, sg_t, \sum_{t}^{t+k}r_i, s_{t+k})$ to $(s_t, g, sg_t, \widehat{r}_{\phi}(s_t,sg_t), s_{t+k})$. Since $\widehat{r}_{\phi}$ does not depend on changing lower primitive behavior, reward relabeling effectively ameliorates non-stationarity in off-policy HRL caused by obsolete rewards. However, since $\widehat{r}_{\phi}$ is learnt from preference based learning, $\widehat{r}_{\phi}$ is itself non-stationary which may lead to training instability. We propose to deal with this issue by employing target networks~\citep{lillicrap2015continuous}, as explained in Section~\ref{sec:target_networks}. \was{Outdated rewards are no longer present in the buffer, but were updates on $\widehat{r}_{\phi}$ performed using rewards generated by outdated policies?}
%
\us{Actually no, see $\widehat{r}_{\phi}$ is updated using PiL reward $r^s$(generated from sparse environment reward), and regularization reward ( which is also updated and so not outdated). Hence, the rewards used to train $\widehat{r}_{\phi}$ only depend on the trajectory taken (and not the outdated policy)}

\subsection{Primitive informed regularization}
\label{primitive_informed_regularization}
As explained above, the preference reward learnt using PiL motivates the higher level policy to reach the goal $g$, while mitigating non-stationarity. However, the higher level subgoal predictions $sg_t$ may be too hard for the current lower primitive, which may lead to degenerate solutions. \was{Nice -- do we have experiments illustrating this, or is this a well-known phenomenon in the literature?} \us{We do have experiments which show that our results improve when we regularize with lower primitive value function. See Figure 1 (Green line is piper(with regularization), Pink is piper without regularization).} Ideally, the higher level policy should produce subgoals at appropriate level of difficulty, according to the subgoal achieving capability of the lower primitive, thereby properly balancing the task split between hierarchical levels. We propose to use the lower primitive state value function $V^{L}(s_t,sg_t)$ to regularize the higher level policy to predict achievable subgoals for the lower level policy. Intuitively, $V^{L}(s_t,sg_t)$ provides an estimate of the achievability of subgoal prediction $sg_t$, since a high value of $V^{L}(s_t,sg_t)$ implies that the lower primitive expects to achieve high reward when $sg_t$ is predicted, based on prior learning.
\par We represent the implicit primitive informed regularization reward $r^v(s_{t},sg_{t})$ as: $r^v(s_{t},sg_{t})=V^{L}(s_{t},sg_{t})$, and compute the sum of $r^{v}$ for higher level behavior sequence $\sigma^{i}$ as: $\sum_{j=0}^{n} r^{v}(s_{t+jk},sg_{t+jk})$. This primitive informed regularization reward motivates the higher level policy to predict achievable subgoals. We augment reward $r^s$ in Equation~\ref{eqn:reward_s} using additional primitive informed regularization reward $r^v$. Formally, for the goal $g$, $\sigma^1 \succ \sigma^2$ when:

\begin{equation}
\label{eqn:reward_total}
    \begin{split}
        \sum_{j=0}^{n} r^{total}(s_{t+jk}^{1},g,sg_{t+jk}^{1}) > \sum_{j=0}^{n} r^{total}(s_{t+jk}^{2},g,sg_{t+jk}^{2})
    \end{split}
\end{equation}
where $r^{total}(s_j,g,sg_j) = r^{s} (s_j,g,sg_j) + \alpha * r^{v} (s_j,sg_j)$, and $\alpha$ is weight parameter for primitive informed regularization reward. The preferences elicited using $r^{total}$ are subsequently used to learn the preference reward function $\widehat{r}_{\phi}$, which in turn is used to relabel higher level off-policy replay buffer transitions. Thus, PiL and primitive informed regularization mitigates non-stationarity, while regularizing the higher policy to predict achievable subgoals for the lower primitive. Notably, since $V^{L}$ is used to relabel the experience previously seen during training, the over-estimation issue of state value function $V^{L}$ on out-of-distribution states does not arise.

\subsection{Goal-conditioned hindsight relabeling}
\label{sec:hr}
The PiL feedback reward $r^{s}$ learnt in Section~\ref{section:pil} is used to elicit preference among higher level behavior sequences, as shown in Equation~\ref{eqn:reward_total}. However, since $r^{s}$ is sparse, it mostly fails to generate a meaningful reward signal, especially during initial training phase. Consequently, $r^{s}$ is unable to generate appropriate preference signal, when comparing higher level behavior trajectories.
\par In order to deal with sparse reward issue, we employ hindsight relabeling~\citep{andrychowicz2017hindsight} to relabel the goal when comparing trajectories $\sigma^{1}$ and $\sigma^{2}$. Concretely, we first sample an achieved state from trajectories $\sigma^{1}$ and $\sigma^{2}$ as the new goal $\widehat{g}$: that is $\widehat{g} \sim \{s_{t+jk}^{1}| j \in (1,2,...n) \} \cup \{s_{t+jk}^{2}| j \in (1,2,...n) \} $, and then compute Equation~\ref{eqn:reward_total} by replacing $g$ with $\widehat{g}$. Formally, for the hindsight relabeled goal $\widehat{g}$, $\sigma^1 \succ \sigma^2$ when:

\begin{equation}
\label{eqn:hindsight_relabeling}
    \begin{split}
        \sum_{j=0}^{n} r^{total}(s_{t+jk}^{1},\widehat{g},sg_{t+jk}^{1}) > \sum_{j=0}^{n} r^{total}(s_{t+jk}^{2},\widehat{g},sg_{t+jk}^{2})
    \end{split}
\end{equation}
where $r^{total}(s_j,\widehat{g},sg_j) = r^{s} (s_j,\widehat{g},sg_j) + \alpha * r^{v} (s_j,sg_j)$. Using hindsight relabeling, the policy is able to generate significantly better preference feedback with improved sample efficiency. We show in Section~\ref{sec:experiments} that this simple hindsight relabeling approach significantly boosts performance in complex sparse reward tasks.

\subsection{Reward stabilization via target networks}
\label{sec:target_networks}
The reward model $\widehat{r}_{\phi}$ is learnt using preference based learning, which may cause training instability due to non-stationary rewards $\widehat{r}_{\phi}$. Another preference based learning approach PEBBLE~\cite{DBLP:journals/corr/abs-2106-05091} deals with this issue by relabeling all the replay buffer transitions every time the reward $\widehat{r}_{\phi}$ is updated. In contrast, we propose to deal with this issue by utilizing target reward model with soft target updates~\citep{lillicrap2015continuous} to provide consistent targets. We create a copy of reward model as $\widehat{r}_{\phi^{'}}$, which is used to calculate target values. We perform soft target updates to the weights of target network: $\phi{'} \leftarrow \tau \phi + (1-\tau)\phi{'}$ where $\tau \ll 1$. In practice, we found that this mitigates reward model non-stationarity and greatly stabilizes learning.

\par We explain our approach in detail in Algorithm~\ref{alg:algo_piper}. The higher level and lower level policies are both trained using Soft Actor Critic (SAC)~\citep{DBLP:journals/corr/abs-1801-01290}. The rewards in higher level transitions are relabeled using the reward model $\widehat{r}_{\phi}$. Instead of relabeling all replay buffer transitions, we relabel the higher level replay buffer transitions as they are sampled while training, as explained in Algorithm~\ref{alg:algo_piper}.

\begin{algorithm}[H]
\caption{PIPER}
\label{alg:algo_piper}
\begin{algorithmic}[1]
    % \Require $D, Q_{th}$
    \STATE Initialize preference dataset $D = \{\}$
    \STATE Initialize higher level replay buffer $\mathcal{R}^{H} = \{\}$ and lower level replay buffer $\mathcal{R}^{L} = \{\}$
    \STATE Initialize reward model parameters of $\widehat{r}_{\phi}$
    \STATE Initialize target reward model parameters of $\widehat{r}_{\phi^{'}} \leftarrow \widehat{r}_{\phi}$
    \FOR{$i = 1 \ldots N $}
        \STATE // Collect experience using $\pi^{H}$ and $\pi^{L}$ and store transitions in $\mathcal{R}^{H}$ and $\mathcal{R}^{L}$
        \FOR{each timestep $t$}
            \STATE $d^{H} \leftarrow d^{H} \cup \{(s_t, g, sg_t, \sum_{t}^{t+k}r_i, s_{t+k})\}$
            \STATE $d^{L} \leftarrow d^{L} \cup \{(s_t, sg_t, a_t, r_t, s_{t+1})\}$
        \ENDFOR
        \STATE $\mathcal{R}^{H} \leftarrow \mathcal{R}^{H} \cup d^{H}$
        \STATE $\mathcal{R}^{L} \leftarrow \mathcal{R}^{L} \cup d^{L}$
        \STATE // Sample higher level behavior trajectories and goal
        \STATE $(\sigma^{1}, \sigma^{2}) \sim \mathcal{R^{H}}$ and $g \sim \mathcal{G}$
        \STATE Sample a set of additional goals for relabeling $\mathcal{G^{'}}$
        \FOR{$g^{'} \in \mathcal{G^{'}}$}
            \STATE Relabel $g$ by $g^{'}$ and generate label $y$ using Equation~\ref{eqn:hindsight_relabeling}
            \STATE Store preference $\mathcal{D} \leftarrow \mathcal{D} \cup \{(\sigma^{1}, \sigma^{2}, y)\}$
        \ENDFOR
        \STATE // Reward Model Learning
        \FOR{each gradient step}
            \STATE Optimize model reward $\widehat{r}_{\phi}$ using Equation~\ref{eqn:reward_cross_entropy}
            \STATE // Update target reward model parameters
            \STATE $\phi{'}_{\widehat{r}} \leftarrow \tau \phi_{\widehat{r}} + (1-\tau)\phi{'}_{\widehat{r}}$
        \ENDFOR
        \STATE // Policy Learning
        \FOR{each gradient step}
            \STATE Sample $\{(\sigma_j)\}_{j=1}^{m}$ from $\mathcal{R}^{H}$ and $\{(\delta_j)\}_{j=1}^{m}$ from $\mathcal{R}^{L}$
            \STATE Relabel rewards in $\{(\sigma_j)\}_{j=1}^{m}$ using target reward model $\widehat{r}_{\phi^{'}}$
            \STATE Optimize higher policy $\pi^{H}$ using SAC
            \STATE Optimize lower policy $\pi^{L}$ using SAC
        \ENDFOR
    \ENDFOR
\end{algorithmic}
\end{algorithm}
